Vidur: A Large-Scale Simulation Framework For LLM Inference

Optimizing the deployment of Large language models (LLMs) is expensive today since it requires experimentally running an application workload against an LLM implementation while exploring large configuration space formed by system knobs such as parallelization strategies, batching techniques, and scheduling policies. To address this challenge, we present Vidur - a large-scale, high-fidelity, easily-extensible simulation framework for LLM inference performance. Vidur models the performance of LLM operators using a combination of experimental profiling and predictive modeling, and evaluates the end-to-end inference performance for different workloads by estimating several metrics of interest such as latency and throughput. We validate the fidelity of Vidur on several LLMs and show that it estimates inference latency with less than 9% error across the range. Further, we present Vidur-Search, a configuration search tool that helps optimize LLM deployment. Vidur-Search uses Vidur to automatically identify the most cost-effective deployment configuration that meets application performance constraints. For example, Vidur-Search finds the best deployment configuration for LLaMA2-70B in one hour on a CPU machine, in contrast to a deployment-based exploration which would require 42K GPU hours - costing ~218K dollars. Source code for Vidur is available at https://github.com/microsoft/vidur.

==> 3-motivation.tex <==
\section{Motivation}
\label{sec-mot}


==> figures-tex/fig-dominant-features.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.4]{graphs/70b_chat_dominant_features.pdf}
    \caption{\small
        Spider chart illustrating the role of individual configuration parameters in optimizing latency metrics. Analysis on \llamaL for \chat workload. Each hexagon represents a specific metric we are interested (e.g. TTFT-P50). Each corner in the hexagon represents a parameter in the deployment configuration, eg., TP dimension, batch size, etc. 
    Each parameter is plotted on the spider chart with distance from center and size proportional to the frequency of the feature in points on or near the Pareto frontier. Points futher away from the center represent the dominant choices that are made most frequently. A clustering of small points close to the center indicates relative insignifiance of the configuration choice. 
    }
    \vspace{-0.2in}
    \label{fig-dom-feat}
\end{figure*}


==> figures-tex/fig-fidelity-bar.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.55]{graphs/fidelity_runtimes.pdf}
    \caption{Comparing fidelity of \sysname predictions for large scale deployment runs across 32 A100 GPUs for \chat}
    \label{fig-scale-fid}
    \vspace{-12pt}
\end{figure*}


==> figures-tex/fig-scheduler-whatif-latency-lmsys.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.7]{graphs/sched_whatif_capacity_vs_piecewise_latency_chat.pdf}
    \caption{What-if analysis with varying scheduling policies.}    
    \label{fig-whatif-scheduler-latency}
\end{figure*}


==> figures-tex/fig-tp-whatif-latency-lmsys.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.7]{graphs/tp_whatif_capacity_vs_piecewise_latency_chat.pdf}
    \caption{What-if analysis with varying tensor parallel dimensions. We vary TP dimension as 1, 2 and 4 keeping the batch size as 64.}
    \label{fig-whatif-tp}
\end{figure*}


==> tables/eval-e2e-stats.tex <==

 



\begin{table*}[]
\center
\scalebox{0.85}{
\begin{tabular}{c|ccc|ccc|ccc|clll} \hline
\multirow{2}{*}{Dataset}   & \multicolumn{9}{|c|}{Request execution time (s)}  & \multicolumn{3}{|c}{Exp time (min)} \\ \cline{2-13}

 & \multicolumn{3}{|c|}{Median} & \multicolumn{3}{|c|}{p75} & \multicolumn{3}{|c|}{p90} \\ \cline{2-12}
 & \sysname & Dep & Error & \sysname & Dep & Error & \sysname & Dep & Error & \sysname & Dep \\ \hline
 
LLaMA2-7B (TP-1) & 1.78	& 1.74 & +2.30\% & 4.04 & 3.95 & +2.28\% & 6.28 & 6.16 & +1.95\% & 0.5 & 12.5   \\ 
LLaMA2-34B (TP-2) & 5.47 & 5.6 & -2.32\% & 12.25 & 12.64 & -3.09\% & 18.78 & 19.29 & -2.64\% & 0.5 & 13.1 \\
LLaMA2-70B (TP-4) & 22.97 &	22.86 & +0.48\% & 50.84 & 51.11 & -0.53\% & 77.77 & 78.44 & -0.85\% & 0.5 & 14.5 \\
\hline

\end{tabular}}
\caption{Comparing large scale deployment runs across 32 A100 GPUs with \sysname}
\label{tbl-eval-e2e-stats}
\end{table*}


==> tables/eval_setup.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}{ccccc} \hline
Model & GPU & Tensor Parallel Size\\
\hline
LLaMA2-7B & A40/A100 & 1 \\
LlaMA2-34B & A100 & 2 \\
LlaMa2-70B & A100 & 4 \\
\bottomrule
\end{tabular}
\caption{Models and their default cluster configurations used for evaluation.}
\label{tbl-eval-setup}
\end{table}

